EgoThink: Evaluating First-Person Perspective Thinking Capability of Vision-Language Models

Vision-language models (VLMs) have recently shown promising results in traditional downstream tasks. Evaluation studies have emerged to assess their abilities, with the majority focusing on the third-person perspective, and only a few addressing specific tasks from the first-person perspective. However, the capability of VLMs to "think" from a first-person perspective, a crucial attribute for advancing autonomous agents and robotics, remains largely unexplored. To bridge this research gap, we introduce EgoThink, a novel visual question-answering benchmark that encompasses six core capabilities with twelve detailed dimensions. The benchmark is constructed using selected clips from egocentric videos, with manually annotated question-answer pairs containing first-person information. To comprehensively assess VLMs, we evaluate eighteen popular VLMs on EgoThink. Moreover, given the open-ended format of the answers, we use GPT-4 as the automatic judge to compute single-answer grading. Experimental results indicate that although GPT-4V leads in numerous dimensions, all evaluated VLMs still possess considerable potential for improvement in first-person perspective tasks. Meanwhile, enlarging the number of trainable parameters has the most significant impact on model performance on EgoThink. In conclusion, EgoThink serves as a valuable addition to existing evaluation benchmarks for VLMs, providing an indispensable resource for future research in the realm of embodied artificial intelligence and robotics.

==> sec/5_evaluation.tex <==
\section{Evaluation Method}




To assess the visual-language capabilities, evaluating open-ended model generations is not a trivial problem. Firstly, no restrictions are applied to model generations in our setting to fit diverse questions. This means model generations and reference answers may have very different formats but the same meaning. Hence, match-based metrics, such as accuracy, F1 scores, and exact match, are not suitable anymore. Furthermore, question types are very diverse in a real-world environment and reference answers may not be the only correct ones. For example, in planning questions, more than one feasible route can exist, and they may be essentially different. Therefore, similarity-based metrics such as BLEU~\citep{papineni-etal-2002-bleu} and ROUGE~\citep{lin-2004-rouge} are ineffective for these questions.
To tackle these challenges, following~\citet{zheng2023judging}, we propose to use GPT-4~\citep{openai2023gpt4} as the automatic evaluator to better measure generated answers under the open-ended setup. Specifically speaking, we design two types of evaluation protocols: reference-guided grading and pairwise comparison.

\vspace{2pt}
\noindent\textbf{Single-answer grading.} In this protocol, we want to measure how close one model output is to the reference. Different from traditional similarity-based methods, GPT-4 pays more attention to semantics. This means even if the model output is different from the reference in wording or syntax, the score is still reliable as long as they mean the same thing. In the detailed implementation, we format the question, the model output, and the reference in a prompt (\todo APPENDIX HERE) and feed it into the GPT-4 evaluator. The GPT-4 evaluator is asked to assign a score between 1 and 10 to the model output. (\todo ACTUAL SCORE).

% \vspace{2pt}
% \noindent\textbf{Pairwise Comparison.} Single-answer grading is not always reliable as exact grades provided by GPT-4 are less interpretable. Therefore, a pairwise comparison is easier for the GPT-4 evaluator and thus more interpretable and reliable. In this case, provided with the question, the reference, the model output, and an anchor answer, GPT-4 is required to judge whether the model output or the anchor answer is better. (\todo APPENDIX HERE) In our experiment, we use the output of GPT-3.5 with a captioner as the consistent baseline to generate the anchor answer. 
% Furthermore, considering the positional bias problem, we exchange the positions of the evaluated model and the baseline across two runs.
% The output of the GPT-4 evaluator is either 0 or 1 score, indicating the evaluated model or the baseline is better respectively. 
% We then compute the final score as the average of the two runs.
